Evaluating Chatbots to Promote Users' Trust -- Practices and Open Problems

Chatbots, the common moniker for collaborative assistants, are Artificial Intelligence (AI) software that enables people to naturally interact with them to get tasks done. Although chatbots have been studied since the dawn of AI, they have particularly caught the imagination of the public and businesses since the launch of easy-to-use and general-purpose Large Language Model-based chatbots like ChatGPT. As businesses look towards chatbots as a potential technology to engage users, who may be end customers, suppliers, or even their own employees, proper testing of chatbots is important to address and mitigate issues of trust related to service or product performance, user satisfaction and long-term unintended consequences for society. This paper reviews current practices for chatbot testing, identifies gaps as open problems in pursuit of user trust, and outlines a path forward.

==> attempt-compute-survery/sec1_introduction.tex <==
\section{Introduction}

A chatbot is a computer program employing artificial intelligence (AI) methods to  interact with humans in natural language. While the simplest setting of a chatbot is a user interacting with the system using text for chit chat, in the most general case, one or more users can interact with the system using text, voice (audio) and image/ videos and the system can respond similarly, thereby collaboratively accomplishing user(s) goals. 


In this paper, we consider chatbots in the context of business applications and survey techniques  to test them to promote user's trust. Trust is a multi-faceted quality that is studied in the context of humans in humanities, and now increasingly gaining importance in AI as systems and humans collaborate closely. In \cite{trust-ml-book}, the author identifies  a trustworthy machine learning system as one that can demonstrate sufficient competence (basic performance), reliability, support for human interaction and alignment with human purpose. For our chatbot purpose, we will consider the first three - competence, reliability and human interaction.

The testing of a chatbot can be considered sufficient on the basis of testing baselines for software systems like unit, system, integration and regression tests. They can also be considered sufficient based on baselines for AI systems like data diversity, model performance (like accuracy, recall, F1 score). Finally, they can also be considered sufficient based on baselines for decision support systems which work with humans like randomized control trials (RCT), Net Promoter Score (NPS), focus groups and customer feedbacks. We will consider a mix of these for chatbot testing. 

\subsection{Chatbots in Business}



% \begin{enumerate}
%     \item Businesses are looking towards digital services

    
%     \item Chatbot as a way for engaging users - both customers, vendors and employees,

%     \item Open question about effectiveness and trust. 

%     \item Paper is about chatbot testing which can help with user trust.

%     \item Outline of the paper
% \end{enumerate}
% ----
%\subsection{Businesses are going digital}

Digital services are becoming increasingly popular among businesses for a variety of reasons. They can be flexibly adapted and tailored to the specific needs of customers, reach a wider audience beyond geo-physical boundaries, and be more engaging and interactive. These can also be more cost-effective than traditional methods, and can be updated more easily and quickly.
% These can be more cost-effective than traditional methods, reach a wider audience, and be more engaging and interactive. 
% Additionally, digital services can be more flexible and tailored to the specific needs of a business, and can be updated more easily and quickly.

A  popular form of digital service offered by companies is the \textbf{digital sales channel}. It is an online sales platform that enables businesses to reach and sell to customers through the use of the internet. There are many different types of digital sales channels, such as virtual sales agents, online marketplaces, and social media platforms. Each type of digital sales channel has its own unique advantages and disadvantages that businesses must consider when deciding which channel is right for them. 
Digital sales channels lay within the broader concept of digital marketing which involves applications of digital technologies which form online channels to market, such as web, email, databases, but also mobile and wireless channels and digital TV \cite{chaffey2009internet}.

% \subsection{Businesses deploy chatbots to engage with their target groups}

Chatbots are a great way to engage users. By providing a way for users to communicate with a chatbot, businesses can provide interactive experience that keeps users engaged. Additionally, chatbots can provide a way for users to get information or perform tasks without having to leave the site or app. This can be particularly useful for tasks that are time-consuming or repetitive. 

Businesses may design and deploy chatbots to engage more than one target group of users. Company's customers, vendors, employees and even the public, as often represented by the local community - all may need to be addressed and served by the chatbot. In addition to considering the target group, the design of the chatbot should take into account the specificities of the channel it is meant to address, such as whether it is a text-based or voice-based channel. The design should also ensure that the chatbot is able to answer the different types of queries by different stakeholders that may be directed to it. The success of a chatbot in addressing the needs of its target audience depends on the level of trust that users have on the chatbot. In order for a chatbot to be successful, it is important that users trust the chatbot and believe that it will be able to help them. One of the ways to build trust is to ensure that the chatbot is designed to be transparent and honest with its users.

% In this paper, we focus on the \textbf{conversational agents}, that 
Chatbots become the digital link between the consumer and the company selling the products or services. We mostly address agents from the perspective of customer support. There are several types of consumer oriented virtual agents. To highlight different dimensions of consumer trust, in this paper we mostly think of three types of consumers: streaming service, medical advice service and property sales. Virtual agents may be differentiated by the trust associated dimensions, such as accuracy, language, ethics and other.

\textbf{Virtual sales agents} are a type of digital sales channel that can be used to reach and sell to customers online. Virtual sales agents are automated software programs that are designed to simulate the experience of interacting with a human sales agent. Virtual sales agents interact with customers and provide them with information about a company’s products or services. They can be used to provide customer service, generate leads, and close sales. One of the advantages of using virtual sales agents is that they are available 24/7 and can scale to meet the needs of businesses of all sizes. While they may not be human, businesses are hoping that they will be able to provide consumers with the same level of trust that they would expect from a real salesperson.



% (WHAT'S THIS PAPER ABOUT)
Chatbot is not a human being, hence not subject to the protocols of human interaction, such as in classic understandings of customer engagement or human resources. Characterizing trust in user-chatbot interaction needs novel approaches. This paper discusses the issues of user trust towards chatbots and if chatbot testing can help with user trust. The first chapter provides an overview lays out the environment for the issues of chatbot trust. Key concepts are briefly explained, including digital platforms, digital sales channels, chatbot usage in business settings, virtual sales agents, effectiveness of virtual agents and issues of consumer trust. Overview of the authors previous studies in building chatbots follows. Chatbots of different functions are introduced: 1) a multi-modal educational Rubik's cube chatbot, 2) natural language to structured query (NL2SQL) system, 3) university chatbot and 4) planning chatbot.

In section two, we provide an overview of the terminology and characteristics of business processes in the context of virtual agents. This provides an introduction to the needs and methods for testing chatbots. The need for consumer trust in chatbots is highlighted. Chatbot testing is discussed in section three, where software testing and comparative studies are discussed. The problems of trust related to chatbot under performance is presented. Section four presents three chatbot usage scenarios highlighting unique testing needs for different types of chatbots. Streaming service, medical advice and property sales chatbots are brought as chatbot example applications.

In Figure~\ref{fig:business-setting}, we illustrate the usage of a chatbot in a business setting covering any number of company's products and services. The chatbot is integrated into the company's IT platform which provides an interface for users interaction. Chatbots are designed and launched by the developers who are often hired on a subcontract basis from outside of the company. Chatbots may serve two categories of users - internal and external. Internal users, for example may be the administrators, such as sales staff who receive sales orders and process these. In a business setting, external users are typically company's customers who use chatbot to acquire information about the products and services, but also to submit orders and receive updates about the order. An advanced chatbot processes also customer feedback, complaints and returns.
% -----------------------------------------
 
\begin{figure}[h]
 \centering
   \includegraphics[width=0.7\textwidth]{content/figs/business-chatbot-setting.png}  
   \caption{Chatbot users in a business setting}
   %shown as a decision tree. }
  \label{fig:business-setting}
 \end{figure}
% -----------------------------------------

%\cite{chatbot-testing-tips,chabot-generator} 


\begin{table}[t!]
%\scriptsize
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Chatbot} & \textbf{Domain} & \textbf{Testing Method} & \textbf{Tool Used}  & \textbf{Details}  \\ \hline
ALLURE & Teaching Rubic's Cube (education) & User study & RASA &  \href{https://youtu.be/-0aKDVoEGvs}{Demo},  \cite{allure}
\\ \hline
NL2SQL Bot & Home network (REZERV) /power (MIDAS) info & NA & RASA  & \href{https://vimeo.com/651270271}{Demo},  \cite{t4}
\\ \hline
UniBot & University info & RCTs & RASA & NA 
\\ \hline
PRUDENT & Information retrieval with planning & Unit testing & ParlAI & 
\\ \hline
ElectionBot & Voter information / elections & Focus group & RASA & 
\\ \hline

\end{tabular}
\caption{Different chatbots we built, their domain, testing method, tool used, demonstration link and the relevant papers.}
\label{tab:uofsc-chatbots}
\end{table}

% ------
\subsection{Our Experience in Building Chatbots and Testing Practices Used}

We describe some of the chatbots we have built in different domains and testing methods used.  Table \ref{tab:uofsc-chatbots} gives a summary. 
%We also discuss the testing methods we used to evaluate these chatbots.



% -----
%\subsubsection{Education Chatbot} 
ALLURE \cite{allure} is a multi-modal, collaborative, explainable educational chatbot that is designed to help students to improve their problem solving skills by teaching them how to solve a Rubik's Cube. The chatbot interacts with the users in a multi-modal way by making use of both text and image modalities. It converts output from the black-box Deep Reinforcement Learning (RL) algorithm in the back-end to a human-understandable language and also demonstrates the set of moves the users have to perform using a 3D model of the Rubik's cube on the User Interface (UI). We used RASA \cite{rasa} chatbot framework to build the chatbot and used React JS framework to build the UI around the chatbot. A demo of the system can be found \href{https://youtu.be/-0aKDVoEGvs}{here}. We have conducted a user study to evaluate the chatbot. \kl{Need to add more details about user study.}

%\subsubsection{NL2SQL Chatbot}
NL2SQL chatbot - in \cite{t4}, we built a rule-based natural language to structured query (NL2SQL) system which could convert the Natural Language (NL) query from the user to a MySQL query and fetch the relevant data from the back-end databases. We created a chatbot around this system and implemented it in two different domains with different settings: 
% \begin{itemize}
%     \item 
    {\em Networking:} We used router data in a residence setting. All the internet devices are connected to a smart router that stores and pushes network activity data to the database. 
    %\item 
    {\em Power:} We used IoT power sensor data in a University setting. An electronic sensor is placed in the path of the power source of each device connected to the IoT and data like current and power are captured and pushed to a database. Data was collected from about 100 servers.
%\end{itemize}
We used RASA \cite{rasa} chatbot framework to build the chatbot and deployed it on the Alexa device and a local server for demonstration which can be found \href{https://vimeo.com/651270271}{here}.

\bips{Kausik, put links in Table and describe based on group webpage.}
% \subsubsection{University Chatbot}
% \kl{Need info.}
% \subsubsection{Planning Chatbot}


% \kl{Need info. - Biplav}


==> attempt-compute-survery/sec2_background.tex <==
\section{Background}

In this section, we ground the terminology and characteristics of business processes and technology in the context of virtual agents, so that the needs and methods for testing can be better understood.



% -------
\subsection{What are chatbots?}

A chatbot is a computer program that simulates human conversation. It uses artificial intelligence to understand and respond to questions in natural language. Chatbots can range from simple to complex, but most chatbots are designed to perform a specific task, such as customer service or sales.
A simple taxonomy of interaction interfaces we consider {\bf chatbot} for the purpose of the paper is shown in Table~\ref{tab:chatbot-types} under {\em Dimension} column. The {\em users} of the system can be single or a group. As interaction {\em modality}, one can talk to a system or, if speech is not supported, type an input and get the system's response. The system may be for different {\em purposes}: converse in pleasantries without a goal (socialize) and with no need to access data sources, or complete a task like retrieve information or take an action.
To do so, the system can be connected to a static {\em data source} like a company directory or a dynamic data source like disease cases or weather forecast. The application scenarios become more  compelling when the chatbot works in a dynamic environment, e.g., with sensor data,  interacts with groups of people who come and go rather than only an individual at a time, and adapts its behavior to peculiarities of user(s). 
The system can be in many {\em forms} - as software that runs as apps on phones and computers, or embedded into   physical artifacts like kiosks, robots, toys, cars or rooms to give a rich user experience. They may be {\em personalized} to users and be customized for different {\em applications} areas.
This variety is illustrated  in the right column of Table~\ref{tab:covid-decsupport}.

% ---------------------

\begin{table}[t!]
%\scriptsize
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{S.No.} & \textbf{Dimension} & \textbf{Variety} \\ \hline
1 & User & 1, multiple \\ \hline
2 & Modality &  only text,  only speech, multi-modal \\ 
  &   & (input with pointing device, output on a map, ...) \\ \hline
3 & Purpose & socialize, (goal driven:) information seeker,  \\ 
  &  & (goal driven:) delegate action  \\ \hline
4 & Data source & none, static, dynamic \\ \hline
5 & Form & virtual agent, physical device, robot \\ \hline
6 & Personalized &  no, yes \\ \hline

7 &  Domains & general, health, water, traffic, ...\\ \hline

\end{tabular}
\caption{Different Types of Collaborative Interfaces}
\label{tab:chatbot-types}
\end{table}
% ---------------------

 
% --------
\subsection{Business Operations and the Role of Chatbots}

In the past decade, there has been a dramatic shift in the way businesses operate. With the rise of the internet and digital technologies, businesses have had to adapt to a new landscape. This has led to the rise of digital business.

\textbf{Digitalization in business} is the process of using digital technologies to create value for the customers. This can be done in a variety of ways, such as a website, a mobile app, social media or by developing a conversational agent to connect with customers.

Conversational agents gain popularity because it allows to reach a larger audience with the product or service. It also allows the business to connect with customers in a more personal way. Additionally, conversational aagent is more cost-effective than traditional methods of marketing and advertising.

As with traditional customer engagement channels, so do digital channels need to be incorporated into company's general and specific strategies. In case of virtual sales agents, \textbf{digital marketing strategies} need to be addressed. \textbf{Digital marketing} is the process of using the internet and digital devices to promote and sell products or services. Virtual sales agents are only one component in the digital marketing toolbox. Other digital tools, such as  email, social media, search engine optimization, and pay-per-click advertising are also commonly used. A company's digital marketing strategy is be designed to help the company to move towards marketing goals. Hence, digital marketing strategies need to be in line with the overall marketing strategy, but also with the general strategy of the business. Usually, virtual sales agents are complementing other marketing channels to offer a wider selection of customer service platforms. Using any of the customer channels, the goal is to create a customer journey that leads to conversions and sales.

\subsubsection{Chatbot stakeholders}

There are a number of stakeholders within the context of digital business using chatbots as shown in table~\ref{tab:stakeholders}. These include the developers and providers of chatbot technology, the businesses that use chatbots to interact with customers, and the customers themselves. Each of these groups has a different set of interests and needs, which must be considered when developing and deploying chatbots.

\begin{table}
  \caption{Stakeholders of digital business using chatbots}
  \label{tab:stakeholders}
  \begin{tabular}{ |p{3cm}|p{10cm}|  }
    \toprule
    Stakeholder & Interests\\
    \midrule
    \ Developers & Need to ensure that their products are effective and easy to use. They also need to ensure that chatbots are compatible with the systems and platforms that businesses use \\
    \ Businesses & Need to ensure that they are providing a good customer experience. They also need to ensure that chatbots are integrated into their systems and processes in a way that is efficient and effective.\\
    \ Customers & Need to be able to easily find and use chatbots, and they need to be able to trust that chatbots will give them the right information.\\
  \bottomrule
\end{tabular}
\end{table}


 
The increasing availability of new digital technologies has dramatically changed the way businesses interact and communicate with customers. Modern chatbots are utilizing advanced technologies such as artificial intelligence, machine learning, robotic process automation to improve customer engagement. The more complicated chatbots become, the more technologies these deploy, all of which need to be adressed and evaluated in their impact on consumers' trust. Complex chatbots can substitute human service agents in many tasks and can deliver a similar customer experience. Chatbots can fulfill tasks of customer service functions, such as give recommendations, accept orders, process payments, manage shipments, help in troubleshooting and many more. In many cases, chatbots can provide a faster and more convenient experience for users than dealing with a human agent.

% --------
\subsubsection{Methods for Building Chatbots} 

We now review some common ways to build chatbots. 

\noindent {\bf Slot based chatbots}

Slot-based chatbots, also called rule-based chatbots are a type of chatbot that relies on predefined slots to extract information from a user. This information can be used to provide the chatbot with a context for the conversation, or to fulfill a user request. For example, a chatbot may use slots to collect information about a user's travel plans, such as their destination, travel dates, and budget.

\noindent {\bf Learning based chatbots}

Chatbots that are learning based are able to provide a more humanlike interaction than those that are not. These chatbots can keep track of a conversation and provide appropriate responses by utilizing artificial intelligence. This allows for a more natural feeling conversation for the user. Additionally, learning based chatbots can get to know the user over time and provide better recommendations or insights based on the user's preferences.
The main difference from rule-based chatbots is that learning based chatbots can understand inquires and commands that are not recorded in the preset database.

\subsubsubsection{Testing Challenges in Different Approaches}

Slot and Learning based





% ----
\subsection{Software Testing}

Software testing is crucial part of software development. The suggested way to do it is by accounting for it throughout the software development life-cycle. At the specification stage, test plan should be created to check the completeness of the requirements. Then {\em unit testing} should be done as each module is getting completed. Subsequently, {\em system testing } is done during  integration is  followed by  testing  for nun-functional requirements before release of the software. 


% ----
\subsection{The Need for Consumer Trust in  Technology and Chatbots}
In the past, companies could get away with being less than transparent because consumers had no way of knowing any better. Today, however, consumers are more informed and have access to more information than ever before. As a result, companies must pay attentions to their operations, how these impact consumer trust.

There are many factors that contribute to consumer trust. One of the most important is \textbf{transparency}. Consumers need to feel that they can trust the brands they purchase from and that those brands have their best interests at heart. Transparency builds trust between the company and the consumer. If the consumer feels like they can trust the company, they are more likely to engage in business. Transparency also helps to create a positive reputation for the company. If consumers know that the company is open and honest, they will be more likely to recommend it to others. The overall perception of transparency helps to build customer loyalty. 

Chatbots are a way to build consumer trust because they provide an instant, personal connection with the company, including its products and services. Chatbots can answer questions, provide customer support, and even help to elevate the sales of products or services. Chatbots are always there for consumers when they need them and can be trained to address, even to promote the factors of trust, including the transparency.

To make sure if users trust the chatbot, businesses should analyze users profile, which would help avoiding underperformance and shutdown of their chatbot. This can be accomplished, if the
chatbot treats each user based on their corresponding personality profile \cite{muller2019chatbot}.

Another important factor is \textbf{customer service}. If a brand is responsive to customer feedback and complaints, it shows that they care about their customers and are willing to go the extra mile to ensure their satisfaction.

The image of customer service is largely formed by the interactions between customers and customer service representatives. If these interactions are positive, then the customer is likely to have a positive image of customer service. On the other hand, if the interactions are negative, the customer is likely to have a negative image of customer service. 

Technological innovations, such as chatbot based customer service option, may improve the customer experience, when the system is well designed and complements the existing customer service channels. Where call center phone lines may be overloaded, resulting in long waiting times, a well functional customer service chatbot may handle most of the issues, being available 24/7. 

\textbf{Consistency} is another critical determinant of consumer trust. It is important for brands to be consistent. If a brand is constantly changing its message or products, it can be difficult for consumers to trust that they will be getting what they expect. However, if a brand is consistent in its messaging and delivery, consumers are more likely to trust and continue to purchase from them. This why, conservative consumers may alienate from the brand when radical technological changes are affecting their customer experience - such as taking customer service from phone based to a chatbot based servicing. On the other hand, other customer segments may be attracted by the ease of service, when chatbots are introduced. The company needs to know their customer segments and their corresponding service preferences, to make informed and balanced decisions about digital innovations.


==> attempt-compute-survery/sec3_trust.tex <==
\section{Trust Problems With Chatbots }

\subsection{Problems of trust}
Chatbot trust issues may resemble trust dilemmas as also related to other customer channels. In case of an incompetent human sales agent, poor quality service may only reflect on the work of one person or a specific case. A badly designed chatbot however, may impact the operations of the entire sales channel. When a chatbot is not designed properly, it may give incorrect or misleading information. This could lead to users making bad decisions based on the chatbot's advice. Additionally, chatbots may not be able to keep up with the pace of conversation, leading to frustrating user experiences. Another issue is that chatbots may not be able to understand a user's emotional state, which could lead to the bot responding in an inappropriate way. Shortcomings in data protections measures, when chatbots may collect personal, which could be used for nefarious purposes.

Depending on the design, chatbots may be easily fooled by humans. Chatbots are computer programs that are designed to simulate human conversation. However, a chatbot may be programmed to respond to a certain keyword with a certain response. If a human user says something that includes that keyword, the chatbot will respond with the programmed response, regardless of the context of the conversation. This can lead to confusion and frustration for the users. Additionally, chatbots may also be fooled by humans using spelling or grammar errors, or by humans deliberately trying to confuse the chatbot. Chatbots may also be intentionally programmed to respond in ways that are not helpful or informative. 

\subsection{Factors affecting users' trust}

\textbf{User trust} is a multifaceted issue involving accuracy, privacy and other issues of user engagement with any chatbot. A chatbot may not be able to accurately understand or respond to the user's needs. Additionally, chatbots may not be able to keep user information confidential, which could lead to privacy issues.

As digital platforms become prevalent in business services, companies must be aware of how their digital channels affect consumer trust. Consumers are increasingly likely to research a company and its products online before making a purchase, and their trust in a company can be heavily influenced by their online experiences. A company's digital channels provide an opportunity to build trust with consumers by providing accurate and up-to-date information, being responsive to customer inquiries, and maintaining a strong online presence. Conversely, a company's digital channels can also damage consumer trust if they are neglected or poorly managed. It is therefore essential for companies to carefully consider how their digital channels can impact users' trust.

It is essential for businesses to build trust with their users in order to improve customer loyalty. By establishing trust, businesses can create a loyal customer base that will continue to use their products and services.
Trust towards digital platforms may play a critical role in the operational success of said platforms. In other words, if users don't trust a platform, they're less likely to use it. This could lead to a decrease in usage of the platform and consequent loss of revenues. 
Additionally, user trust is important for platforms because it can help to create and maintain brand loyalty. Users who trust a platform are more likely to be loyal to the brand and recommend it to others.

There are many factors that affect \textbf{consumer trust}. Some of these include the company’s reputation, its transparency, its customer service, and its return policy. Other factors include the company’s communication style, the design of its digital channels, and the reviews that consumers can find online from other consumers. Ultimately, it is up to the consumer to decide how much trust to place in a company. Consumer trust is essential for the success of digital sales channels. When consumers feel they can trust a company, they are more likely to do business with them. This trust can be built through transparency, providing accurate information and delivering on promises. Creating a strong relationship of trust with customers can help ensure long-term success for a company.

An \textbf{effective virtual agent} creates trust in consumers by providing accurate and up-to-date information about the products or services they are interested in. They are also transparent about their company’s policies and procedures, and are quick to respond to any questions or concerns that consumers may have. In addition, virtual agents are typically very personable and easy to communicate with, which helps build rapport and further instills confidence in the consumers they are assisting. Ultimately, by being knowledgeable, responsive, and friendly, virtual agents are able to successfully build trust with consumers, leading to satisfied customers and repeat business.

There are a few key factors that contribute to a \textbf{chatbot's competence}. A chatbot must be able to understand the user's input. This is achieved through natural language processing (NLP). Once the chatbot understands the user's input, it must be able to generate a response that is relevant to the user's inquiry. This requires a knowledge base that the chatbot can draw from to generate an appropriate response.  The more detailed database, the higher is the perceived competence of a chatbot. The more accurate the chatbot is in its understanding of the user input and the more relevant the response, the more trust the user will have in the chatbot.

\subsubsection{Accuracy}
Chatbots are not always accurate. The better trained chatbot, the more accurate performance. However, most chatbots are imperfect in their training and are adequately responding only to a limited number of intents. A chatbot with more intents is able to handle more varied user input. This means that the chatbot can respond to a wider range of user queries, which can be helpful in terms of providing a better user experience. Additionally, a chatbot with more intents is likely to have more training data, which can help to improve the chatbot's performance. Chatbot with more intents is more likely to be able to handle edge cases, which can again improve the user experience.

\subsubsection{Reliability} is another key factor in chatbot effectiveness. Businesses deploying chatbots, are trusting the artificial intelligence to carry out conversations on their behalf. A reliable chatbot is designed and and trained to handle most of users' requests. A chatbot that is designed well will be able to understand human conversation and respond accordingly. It will also be able to handle different types of input, such as natural language, text, and even voice. A chatbot that is well-trained will be able to carry out conversations more smoothly and accurately. It will know how to respond to different types of questions and requests, and it will be able to handle different types of conversations.

\subsubsection{Transparency} is a critical part of reliability directly impacting users' trust. Revealing their artificial identity is a central question for any chatbot and customer interaction. A well integrated chatbot provides a seamless customer experience and improves customer satisfaction. Such a chatbot works in line with other tools and channels as deployed by the company and all aimed at providing a trustworthy experience. A transparent chatbot will reflect the transparency of the business in its dealings with customers, providing them with clear and concise information about its products and services. A transparent company is responsive to customer queries and concerns, and always acts in the best interests of the customer. By adhering to these principles, a company can build a chatbot reflecting this trust with its customers, resulting in a long-lasting relationship of mutual respect and understanding.

\subsubsection{Use of language}
A chatbot might use profanity, make threatening comments, or engage in other forms of verbal abuse. This type of language is not only hurtful, but can also be illegal. Abusive language can have a significant impact on chatbot trust. By using profanity or other offensive language, users can create a negative association with the chatbot that can dissuade others from trusting it. In some cases, abusive language can also lead to chatbot technical issues. As such, it is important to be mindful of the language used when interacting with chatbots, in order to maintain a positive relationship and avoid any potential negative impacts.
Chatbots that use profanity can give users a negative impression of the chatbot and the company or organization that chatbot represents. Additionally, profanity can also be seen as a sign of disrespect towards the users of the chatbot. If chatbots continue to use profanity, it is likely that they will eventually be shut down.

\subsubsection{Response time}
Chatboth's response time and time to reach a resolution can also impact the reliability. When a chatbot is slow to respond and reach a satisfying resolution, this can be a source of frustration for customers who are trying to get help or information. As with any customer service interaction, response time and resolution time are key factors in chatbot reliability and customer satisfaction. If a chatbot is taking too long to respond to queries, or is unable to resolve issues in a timely manner, customers will likely  look for alternatives ways for getting the needed information or reach another form of resolution. On the other hand, chatbots that are able to quickly and efficiently resolve customer issues will foster trust and satisfaction. In order to maximize chatbot reliability and customer satisfaction, businesses should monitor response and resolution times closely, and make improvements as needed.

Studies have shown that people are more likely to trust a technology if it is perceived to be reliable. If chatbots are perceived as unreliable, this could lead to decreased trust in the technology overall. This could have a negative impact on how people view chatbots and could lead to fewer people using them.
Chatbots reliability can be undermined by many ways. Overall, a competent and reliable perception of a chatbot is important for ensuring that its able to carry out conversations effectively and accurately, hence gaining trust of the users. 



==> attempt-compute-survery/sec4_chatbottesting.tex <==

\section{Chatbot Testing Methods}

After launching a chatbot, the company needs to monitor \textbf{ chatbot's performance} and to determine if it's performing optimally and achieving company's goals. From the perspective of users' trust, the chatbots performance is mainly related to its competence and reliability. Performance metering can be done through a variety of methods, such as tracking key metrics, conducting user surveys, and A/B testing. By doing so, the company can identify areas for improvement and make necessary changes to ensure the chatbot is providing the best possible experience for users.

\subsection{Purpose and types of tests}
Chatbot testing is the process of testing a chatbot to ensure it is functioning correctly and providing an accurate and consistent experience for users. By testing, companies can identify any issues that need to be addressed, such as incorrect responses, errors, or slow performance. Testing also allows to fine-tune chatbot's design and functionality, as well as assess its overall effectiveness. This involves testing the chatbot's ability to understand and respond to user input, as well as its overall functionality. Chatbot testing can be performed manually or using automated software testing tools.

Testing may include, assessing how well the chatbot understands customer queries, how accurate the chatbot's responses are, and how satisfied customers are with the chatbot experience. Customer satisfaction is one of the key factors of chatbot effectiveness.

\subsection{Software testing}
Chatbot software testing is an important part of the development process, as it helps to ensure that the chatbot is able to deliver a good user experience. 

Chatbot testing can be approached as any other software testing. These methods include unit testing, integration testing, system testing, and acceptance testing. Unit testing is the testing of individual chatbot components, while integration testing is the testing of how those components work together. System testing is a more holistic approach that tests the entire system, including the connections to databases, such as customer, orders, inventory and other. 

Chatbot software testing is essential to ensure that chatbot functions as intended and provides a positive experience for users. Chatbot functional testing ensures that the chatbot is able to handle all the different types of input that it may receive and provide the appropriate responses. Load testing ensures that the chatbot can handle high volumes of traffic without experiencing any issues.

\subsection{Testing as Software Systems}

\subsection{Testing as AI}

\subsubsection{Data sources and provenance}

Data provenance is the origin of data and the history of how it has been transformed over time. Data provenance is often used to track the origins of data, to ensure that it has not been tampered with, and to verify its accuracy. In many cases, data provenance can be used to trace the path of data from its inception to its current form.

As chatbots increasingly become relied upon to handle larger amounts of data, data provenance will become an increasingly important factor in their design and function. Data provenance refers to the origin and history of data, and how it has been transformed over time. For chatbots, data provenance affects how they handle data, what data they have access to, and how that data is used.

Chatbots rely on data to function. If the data they are using is of poor quality or unreliable, the chatbot will be less effective. Data provenance can affect the chatbot’s decision-making. If the chatbot is not aware of the provenance of the data it is using, it may make decisions that are not in the best interest of the user. 

\subsubsection{Large language models (LLMs)}

Large language models (LLMs) are a type of artificial intelligence that are used to process and understand natural language. These are neural networks that are trained on a very large corpus of text. The models are able to learn the statistical properties of the language and can generate text that sounds like it was written by a native speaker. The models are also very good at understanding the context of a sentence, which allows them to generate more natural sounding text. For example, if you ask a chatbot about the weather, it can provide you with information about the current weather conditions as well as the forecast for the next few days.
LLMs can be used for a variety of tasks, including machine translation, question answering, and text classification.

\subsection{Testing as a Decision Support Tools (Comparative Studies)}
Comparative studies are a form of usability testing that assesses how easy it is for users to interact with the chatbot. A comparative study is a effectiveness determination method that observes, if needed, intervenes and compares two or more subsamples, to to identify similarities and differences. This research method can be used to compare anything from individuals to entire organizations. When conducting a comparative study, it is important to control for as many variables as possible in order to create a fair comparison. Once the data is collected, it must be analyzed in order to identify any patterns or trends.
The most reliable way to test the effectiveness of a chatbot is through comparative studies. The most commonly used forms of comparative studies are before/after, case-control, A/B testing and randomized control trials (RCT). There are some important differences between these two types of study designs. A/B testing is designed to test which chatbot works best, while a randomized control trial looks at why it works best. 
In this study we discuss two afore mentioned testing methods, as these are most commonly used and are most advanced and reliable methods for testing for trust.

\subsubsection{A/B testing}
A/B testing is a method of experimentation in which two versions of a chatbot are shown to users at random, and statistical analysis is used to determine which version is more effective. This technique can be used to test anything from chatbot copy to virtual agents capable fullfilling all the tasks of human agents. It also can be used to evaluate how effective a chatbot or virtual agent is in comparison to human agent.
This technique is especially useful when testing or evaluating chatbots because it can help isolate the specific areas where the chatbot falls short. For example, if a chatbot is not able to properly handle customer inquiries, this technique can help identify that particular issue. Additionally, this technique can also be used to evaluate how well a chatbot or virtual agent performs in comparison to human agents.

\subsubsection{Randomized controlled trials}
Randomized controlled trials are a type of scientific experiment that are used to test the effectiveness of a new treatment or intervention. For example, a treatment is a new chatbot, whereas a control is an old chatbot. Industries' best standard or a competitors chatbot could also serve as a control. Additionally, the company to compare a chatbot against other information acquisition channels, such as customer service call center.  The participants in a randomized controlled trial are randomly assigned to either the group receiving the new treatment (a new chatbot) or the control group receiving the standard treatment (an old chatbot). The two groups are then compared to see if the new treatment is more effective. Randomized controlled trials are considered the gold standard of scientific evidence. However, in the case of chatbots, there is a lack of high-quality evidence to support claims of effectiveness, as most chatbot studies do not deploy RCT. RCT is a resource demanding study method that requires time money and often a large number of human test subjects. A recent systematic review found that only two out of eleven studies meets the criteria for an acceptable randomized controlled trial. The other nine studies were either non-randomized or had important methodological flaws. 





==> attempt-compute-survery/sec5_testing_commplatform.tex <==
\section{Case Study: Chatbot Testing Support in Open and Commercial Platforms}


\subsection{Review of Current Practices}

\bips{Nice if we can have a table with references to testing guidance from different vendors. Open Source - parl.ai, rasa, mindmeld.
Keywords: testing, testing guidelines, development process, release checklist}
Chatbots are built for control. Not data-driven ?


\subsubsection{Testing in Watson}
\bips{Sachin - please add based on IBM platform over the years, and coming up.}

\subsubsection{Testing in Rasa}

\subsubsection{Testing in ChatGPT}


\subsection{Testing for Intent Detection}

\begin{itemize}
    \item Handling out-of-scope
\end{itemize}

\subsection{Testing for Actions to Be Taken for an Intent}


\subsection{End-to-end Testing}

Some services provide regression but they are not guaranteed for anything.. Botium. 

\subsection{Opportunities to Improve}

Hate Speech detection. 





==> attempt-compute-survery/sec6_usagescenarios.tex <==

\section{Usage Scenarios - Applications and Unique Testing Needs}

In this chapter we focus on three use cases, discussing the characteristics of those and how these affect chatbot's trust-

Table~\ref{tab:freq} is included in the input file; compare the
placement of the table here with the table in the printed output of
this document.

\begin{table}
  \caption{Overview of chatbot use cases and related trust issues}
  \label{tab:freq}
  \begin{tabular}{ |p{2.5cm}|p{2.5cm}|p{2.5cm}|p{6cm}| }
    \toprule
   Use case&Age of the user&Investment&Focus of user trust\\
    \midrule
    \ Streaming service& Adult and adolescent& Low&Mostly related to protecting adolescents from adult content.\\
    \ Medical advice& Adult& Medium&Related to the health and well-being of the patient.\\
    \ Property sales & Adult & High&Related to transparency and objectivity in investment recommendations.\\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Streaming service chatbot}
In the example  of a streaming service, like Netflix, a chatbot helps the user to find the right movie to watch on their subscription platform. It asks the user questions about what categories they like and don't like, and asks for favorite movies, shows. The chatbot recommends movies for the user.

Movie recommendation is probably one of the lowest personal or property liability examples for a chatbot. However, adult content needs to be screened and made inaccessible for adolescents. A trusted movie chatbot would be capable of identifying the age of the user and accounting for that in its movie recommendations. Besides recommending the titles, the chatbot also needs to account for the language, as it should consider the age of the user.

\subsection{Medical advice chatbot}
Medical advice chatbots are becoming increasingly popular as a way to provide quick and easy medical advice. They are typically used to answer basic questions about medical conditions and treatments, and can be accessed through a chat interface on a website or mobile app.

Medical advice chatbots are needed to be powered by AI models, which allows them to understand natural language queries and provide accurate responses. In some cases, chatbots may also be able to provide personalized recommendations based on a user's individual symptoms or health condition.

So far, due to the risk of liability of malpractice, no chatbot is able to substitute  a human doctor. 
Medical chatbots are subject to highest personal liability, as the function of such service would result in an outcome of human health. Such chatbots need to be able carry the functions of a human doctor, including understanding the health history of the patient, dispositions and side effects and accumulative effects of the medicine. When a chatbot that would prescribe medicine would also need to account for the accumulative effect of multiple prescriptions. 

Seitz et al. studied diagnostic conversational agents. They found that interpersonal trust approaches do not fully explain the build up of trust to diagnostic CAs. Communicative aspects are important in chatbot interactions, but users don't expect a CA to fulfil social needs. Transparent handling of information and justifications are important to build up trust since trust mostly arises cognitively while underlying the technical character of agents. Besides afore mentioned, also  more natural conversation can substantially play a role in trust development. The study identified six trust-building factors in diagnostic chatbots - purpose, reliability, interface design, interaction capabilities, transparency and relativization.  \cite{seitz2022can}

\subsection{Property sales chatbot}

A Property Sales chatbot is a chatbot that is designed to help people with the purchase or sale of their property. The chatbot will ask the user questions about their property or the desired property, such as the price range, the location, and the number of bedrooms. The chatbot will then provide the user with a list of potential buyers or estimate the sales price. 
Property chatbot entails a high expenditure, which makes any misinformation given by the chatbot open for a liability claim. High responsibility requires highest levels of trust in the eyes of the users.
Additionally, chatbot may be required to ckeck the buyer's credit score in order to validate the purchase request. A mortage can not be advised by the chatbot if the buyer is likely incapable of servicing the loan.

Mozafari et al. studied chatbot trust with respect to customer retention. They found that if the chatbot is successful in solving customers' issues, disclosing the identity of chatbot will negatively impact customer trust and therefore obstruct retention for highly critical services. Otherwise, for services of less critical nature, chatbot disclosure won't impact trust. The deficit of trust comes from lower perceptions of agent's competence and benevolence. Lowe benevolence is attributed to perceived lower empathy Agents that are disclosed as virtual agents are seen as less knowledgeable. \cite{mozafari2021trust, bhattacherjee2012user}

==> attempt-compute-survery/secx_others.tex <==


\section{Discussion}


\subsection{Additional Content from Intro}


\subsection{Discussion Content}

Chatbot trust is a complex issue which requires correspondingly complex approach. A trusted chatbot should be adaptive to users need and take into account their personal background. 
Müller et al. determined different user profiles of personality traits to indicate their relative differences of their ability to trust chatbots. They identified three basic personality profiles and their relative level of trust - introverted careless distrusting user, conscientious curious trusting user, careless dishonest trusting user. The user profiles should suggest how the chatbot treats users to result in a perceived trust experience.\cite{muller2019chatbot}

Przegalinska et al. recommended companies focusing on three trust-enhancing features: transparency, integrity, explainability. Transparency means sending signals of honesty in communication, and does not deny its status. Agent also needs to be predictable. The trustors (users) expect that an agent, an object of trust, would act consistently in line with past experience. User perceiving  chatbots as predictable, leads to perception of trust towards the chatbot \cite{przegalinska2019bot}.

What more is needed

\section{Conclusion}

In order to motivate a chatbot for customer interaction it is important to keep the \textbf{chatbot's goals} in mind and make sure that they are aligned with the company's goals. This is is best done before designing a chatbot. Any chatbot's goals should match with  company's goals. Chatbots should be designed to contribute to specific operations and to help the company achieve its desired performance. To do this, first company's specific goals related to the chatbot tasks are identified. These goals are then matched with the features and capabilities of various chatbot strategies. 




==> bio/part1_talk_cv.tex <==
\subsection{Part I: Talk and CV}
% --------------------
\section{Talk Outline }

The proposed talk will survey methods for evaluating collaborative assistants - chatbots - for promoting user(s) trust and engagement, discuss open problems and outline a path forward. We outline  topics to cover that are described in more details in the
attached paper.

\begin{enumerate}
    \item Motivation and vision for a trusted future
    \begin{itemize}
        \item Illustrating trust problem in simple examples
        \item Current development-focused evaluation benchmarks and gaps for gaining user trust
        \item Black-box evaluation settings: no access to code or data
    \end{itemize}
    \item Methods for building chatbots and evaluation considerations
    \item Evaluation methods for chatbots: rule-based, learning-based, LLMs
    \begin{itemize}
        \item As software: unit, system, integration and acceptance testing
        \item As AI: data issues, LLMs
        \item As human-AI collaboration tools: explainability, random control trials (RCTs)
        \end{itemize}
    \item Testing in Practice and Open Problems    \begin{itemize}
        \item  Testing in business
        \item  Testing in healthcare

        \item Open problems
    \end{itemize}

    \item Path Towards Trustworthy Chatbots
        \begin{itemize}
        \item  Modeling chatbots as dynamical systems to use control-theoretic tools for analysis and evaluation
        \item Trust-focused Chatbot Evaluation Framework
        \item User-focused communication of evaluation results

    \end{itemize}
\end{enumerate}

\subsection{Abstract of the Talk}

Chatbots, the common moniker for collaborative assistants, are Artificial Intelligence (AI) software that enable people to naturally interact with them to get tasks done. Although chatbots have been studied since the dawn of AI, they have particularly caught the imagination of the public and businesses  since the launch of easy-to-use and general-purpose Large Language Model-based chatbots like ChatGPT. 
  As businesses look towards chatbots as a potential technology to engage users, who may be end customers, suppliers or even their own employees, proper testing of chatbots is important to address and mitigate issues of trust  related to service or product performance, user satisfaction and  long-term unintended consequences for society. This paper reviews current practices for chatbot testing, identifies gaps as open problems in pursuit of user trust, and outlines a path forward.


% --------------------
\section{CV of Biplav Srivastava}


\subsection{Employment History}
\begin{itemize}
    \item 2020-:	Professor,	AI Institute, University of South Carolina, Columbia, SC, USA



    \item 2001-2010: IBM	
   
   \begin{itemize} 
\item 2018-2020:	Distinguished Data Scientist, Master Inventor	IBM Chief Analytics Office, NY, USA

    \item 2016-2018: Research Staff Member, Master Inventor,	IBM T.J. Watson Lab, NY, USA

\item 2009-2016:	Senior Researcher, Master Inventor	IBM Research, New Delhi, India

\item 2007-2009:	Research Staff Member, IBM T.J. Watson Lab, NY, USA

\item 2001-2007:	Research Staff Member	IBM Research, Delhi \& Bangalore, India
   \end{itemize}

\item 2000-2001:	Core Technology Architect, R\&D	Bodha.com, Los Altos, CA, USA

\item 1996-2000:	Senior Staff Engineer, Philips Semi. (VLSI Tech.), Phoenix, USA; 
PhD Scholar,
Arizona State University, USA

\end{itemize}	

 	          


\subsection{Education}
\begin{itemize}
    \item Ph.D.: Arizona State University, Tempe, AZ, USA, 2000. Dissertation Topic: Efficient Planning by Effective Resource Reasoning
    \item M.S.:  Arizona State University, Tempe, AZ, USA, 1996. GPA:4.0/4.0
    \item B.Tech.: Indian Institute of Technology (IIT), B.H.U., India, 1993.  GPA:9.06/10
    \item Micro-MBA: Management module at IBM taught by faculties of top-US MBA schools.
\end{itemize}	
             
\subsection{Research Interests}
He is interested in enabling people to make rational decisions despite real world complexities of poor data, changing goals and limited resources by augmenting their cognitive limitations with technology. His expertise is in Artificial Intelligence, Sustainability and Services, with proven track record of many science firsts and high-impact innovation (\$B+) in global business environment. 
His research initiatives are on 
promoting 
goal-oriented, ethical, human-machine collaboration  via natural interfaces using  
domain and user models, learning and planning. In particular, he has been exploring the role of reasoning (planning) and learning for human-agent dialogs in individual
and group settings. The use cases are (a) explaining large datasets and their insights to people, and (b) embodiment agents
(environment or room) that can track the discussion and intervene to provide decision support to a group of people.

Biplav has been working in AI trust for 
the last four years pursuing ideas in AI testing, rating, randomized control and adversarial
learning. 
He has conducted Randomized Control Trail (RCT) tests in a large-scale business environment to study
impact of AI on workforce (involving ~140m revenue and ~1000 people; July-Dec 2019). Together with collaborators, he has introduced the idea of rating AI systems for bias as a third-party service, built tools and conducted
experiments.
He applies AI and trust techniques in areas of social as well as commercial relevance 
with particular attention to issues of developing countries  (e.g., water, health, 
transportation, and governance).
He lead building of a tool to understand the role of face mask in controlling COVID19 in US which received significant press.

\subsection{Recognition and Awards}

\begin{itemize}
    \item AAAI Senior Member, recognized by Association for Advancement of Artificial Intelligence for significant contributions and service to AI community (Feb 2020)
    \item AAAS Leshner Public Engagement Fellow, 2020-2021 cohort of the American Association for the Advancement of Science Leshner Leadership Institute for Public Engagement with Science, focusing on AI (Feb 2020)
    \item IBM Master Inventor – for outstanding patent activities (2011-2017, 2019-2022)
    \item Represented IBM at Partnership on AI’s Working Group on Fair, Transparent and Accountable AI 
(2018-2020). https://www.partnershiponai.org 
    \item IEEE Senior Member, for technical achievements (Dec 2018)
\end{itemize}

\subsection{Contributions related to the proposed topic}


\begin{itemize}
    \item Tutorial
    
    \begin{itemize}
      \item Tutorial on Trusting AI by Testing and Rating Third Party Offerings, in conjunction with 29th International Joint Conference on Artificial Intelligence (IJCAI 2020), Biplav Srivastava, Francesca Rossi, Yokohoma, Japan, Jan 2021.
    \end{itemize}
    
    \item Rating related papers
    \begin{itemize}

    
    \item  Mariana Bernagozzi, Biplav Srivastava, Francesca Rossi and Sheema Usmani, Gender Bias in Online Language Translators: Visualization, Human Perception, and Bias/Accuracy Trade-offs, IEEE Internet Computing, Special Issue on Sociotechnical Perspectives,  2021  [Visualizing Ethics Rating, User Survey]

    \item  Mariana Bernagozzi, Biplav Srivastava, Francesca Rossi and Sheema Usmani, VEGA: a Virtual Environment for Exploring Gender Bias vs. Accuracy Trade-offs in AI Translation Services, AAAI 2021. [Visualizing Ethics Rating, Demonstration paper]

    \item  Biplav Srivastava, Francesca Rossi, Sheema Usmani, and Mariana Bernagozzi, Personalized Chatbot Trustworthiness Ratings, IEEE Transactions on Technology and Society, 2020.
    %Pre-publication version on Arxiv - https://arxiv.org/abs/2005.10067, 2020. 
    [Chatbot, Trust Rating, Ethics]

    \item  Biplav Srivastava, Francesca Rossi, Rating AI Systems for Bias to Promote Trustable Applications, IBM Journal of Research and Development, 2019. [AI Service Rating, Ethics]

    \item  Biplav Srivastava, Francesca Rossi, Towards Composable Bias Rating of AI Systems, 2018 AI Ethics and Society Conference (AIES 2018), New Orleans, Louisiana, USA, Feb 2-3, 2018. [AI Service Rating, Ethics]
    \end{itemize}
    
    
    \item Closely related work
    \begin{itemize}
    
          \item Biplav Srivastava, Did Chatbots Miss Their 'Apollo Moment'? A Survey of the Potential, Gaps and Lessons from Using Collaboration Assistants During COVID-19, Cell PATTERNS, Aug 2021. 
          %(Preprint on Arxiv: https://arxiv.org/abs/2103.05561, March 2021)
          [Chatbots, COVID]
    
  
        \item 
    
    Andrea Loreggia, Nicholas Mattei, Taher Rahgooy, Francesca Rossi, Biplav Srivastava and Kristen Brent Venable, Making Human-Like Moral Decisions, AIES 2022. [Neuro-Symbolic, Fast Slow AI, Metacognition]
    
    \item Vignesh Narayanan, Brett W. Robertson, Andrea Hickerson, Biplav Srivastava and Bryant W. Smith, Securing social media for seniors from information attacks: Modeling, detecting, intervening, and communicating risks, The Third IEEE International Conference on Cognitive Machine Intelligence (IEEE CogMI), 2021. [Cyberspace, Seniors] 
    
    \item Bryant Chen, Wilka Carvalho, Nathalie Baracaldo, Heiko Ludwig, Benjamin Edwards, Taesung Lee, Ian Molloy, Biplav Srivastava, Detecting Backdoor Attacks on Deep Neural Networks by Activation Clustering, Artificial Intelligence Safety Workshop (SafeAI) at AAAI-2019, Honolulu, USA, Jan 2019. Best Paper at SafeAI 2019 Workshop. [AI-NN, Safety]
\end{itemize}
\end{itemize}

==> bio/part2_paper.tex <==
\newpage

\subsection{Part II: Paper}
% --------------------
\section{Evaluating Chatbots to Promote Users' Trust - Practices and Open Problems}

\noindent {\bf Biplav Srivastava, Kausik Lakkaraju,  Tarmo Koppel, Vignesh Narayanan, Ashish Kundu, Sachindra Joshi} \\

==> content/secx_kausikLLMtest.tex <==

%\subsection{Evaluation of LLMs}

% Large Language Models (LLMs) such as the GPT models \cite{openai2023gpt4} and PaLM \cite{chowdhery2022palm} have greatly transformed the field of Natural Language Understanding (NLU) and Generation (NLG).  The use of these LLMs and their chatbot variants like ChatGPT and Bard in critical domains like education and healthcare has become a matter of debate due to concerns surrounding ethical implications and their impact on the user's decision-making process. As LLMs are becoming more available in the form of chatbots, the reliability of users on these chatbots has been increasing. This calls for a need to rigorously test these LLMs (and their chatbot counterparts), ensuring accuracy, safety, and trustworthiness. In this section, we discuss the evaluation strategies that are being followed to evaluate or test these LLMs for trustworthiness and accuracy along with the challenges in evaluating them. 
% \subsubsection{Current Evaluation Strategies}

% The evaluation strategies can be classified into three major categories based on the aspects they assess:
% \begin{itemize}
%     \item {\bf Bias and fairness evaluation:}  In \cite{nozza-etal-2022-pipelines}, the authors discuss testing methods inspired by software testing where code is continuously pushed into a common repository and tested to ensure the stability of the model. They also discuss the integration of badges, that identify possible social bias issues one might face while using these LLMs, into the development pipeline. In \cite{kocielnik2023autobiastest}, the authors introduce the AutoBiasTest framework for the generation of test datasets with natural sentences using Pre-trained Language Models (PLMs) for social bias testing in PLMs. They performed testing on 15 known biases and found that using larger models generated better sentences that estimated bias present in PLMs with less variance.  
%     \item {\bf Reasoning abilities evaluation:} In \cite{kıcıman2023causal}, the authors explore the idea of using LLMs as a proxy for domain knowledge along with causal methods. In \cite{jin2023large}, the authors take another step forward by introducing a formal task called CORR2CAUSE that focuses on the pure causal inference task of models, which is a knowledge-dependent reasoning skill based on causal inference. They evaluated GPT- and Llama-based LLMs on this task and found out that these LLMs performed poorly on this task. 
%     \item {\bf Performance evaluation:} In \cite{lakkaraju2023can}, the authors evaluated LLM-based chatbots, ChatGPT and Bard, on the task of financial advisement by asking 13 questions representing banking products and the interactions between them that included questions in different languages and dialects. The chatbots need to satisfy certain mathematical constraints in order to answer these queries accurately. They concluded that there are critical gaps in providing reliable and accurate responses. In \cite{jalil2023chatgpt}, the authors tested whether ChatGPT can answer questions related to software testing accurately. They carefully crafted the queries to test the confidence level and also the explanations provided by ChatGPT along with the accuracy of the response.
% \end{itemize}



==> content/secx_others.tex <==


\section{Remove - Discussion}




\subsection{Additional Content from Intro}


\subsection{Discussion Content}

Chatbot trust is a complex issue which requires correspondingly complex approach. A trusted chatbot should be adaptive to users need and take into account their personal background. 
Müller et al. determined different user profiles of personality traits to indicate their relative differences of their ability to trust chatbots. They identified three basic personality profiles and their relative level of trust - introverted careless distrusting user, conscientious curious trusting user, careless dishonest trusting user. The user profiles should suggest how the chatbot treats users to result in a perceived trust experience.\cite{muller2019chatbot}

Przegalinska et al. recommended companies focusing on three trust-enhancing features: transparency, integrity, explainability. Transparency means sending signals of honesty in communication, and does not deny its status. Agent also needs to be predictable. The trustors (users) expect that an agent, an object of trust, would act consistently in line with past experience. User perceiving  chatbots as predictable, leads to perception of trust towards the chatbot \cite{przegalinska2019bot}.

What more is needed

\section{Conclusion}

In order to motivate a chatbot for customer interaction it is important to keep the \textbf{chatbot's goals} in mind and make sure that they are aligned with the company's goals. This is is best done before designing a chatbot. Any chatbot's goals should match with  company's goals. Chatbots should be designed to contribute to specific operations and to help the company achieve its desired performance. To do this, first company's specific goals related to the chatbot tasks are identified. These goals are then matched with the features and capabilities of various chatbot strategies. 




==> zip-for-reference-only/content/sec1_introduction.tex <==
\section{Introduction}

A chatbot is a computer program employing artificial intelligence (AI) methods to  interact with humans in natural language. While the simplest setting of a chatbot is a user interacting with the system using text for chit chat, in the most general case, one or more users can interact with the system using text, voice (audio) and image/ videos and the system can respond similarly, thereby collaboratively accomplishing user(s) goals. 


In this paper, we consider chatbots in the context of business applications and survey techniques  to test them to promote user's trust. Trust is a multi-faceted quality that is studied in the context of humans in humanities, and now increasingly gaining importance in AI as systems and humans collaborate closely. In \cite{trust-ml-book}, the author identifies  a trustworthy machine learning system as one that can demonstrate sufficient competence (basic performance), reliability, support for human interaction and alignment with human purpose. For our chatbot purpose, we will consider the first three - competence, reliability and human interaction.

The testing of a chatbot can be considered sufficient on the basis of testing baselines for software systems like unit, system, integration and regression tests. They can also be considered sufficient based on baselines for AI systems like data diversity, model performance (like accuracy, recall, F1 score). Finally, they can also be considered sufficient based on baselines for decision support systems which work with humans like randomized control trials (RCT), Net Promoter Score (NPS), focus groups and customer feedbacks. We will consider a mix of these for chatbot testing. 

\subsection{Chatbots in Business}



% \begin{enumerate}
%     \item Businesses are looking towards digital services

    
%     \item Chatbot as a way for engaging users - both customers, vendors and employees,

%     \item Open question about effectiveness and trust. 

%     \item Paper is about chatbot testing which can help with user trust.

%     \item Outline of the paper
% \end{enumerate}
% ----
%\subsection{Businesses are going digital}

Digital services are becoming increasingly popular among businesses for a variety of reasons. They can be flexibly adapted and tailored to the specific needs of customers, reach a wider audience beyond geo-physical boundaries, and be more engaging and interactive. These can also be more cost-effective than traditional methods, and can be updated more easily and quickly.
% These can be more cost-effective than traditional methods, reach a wider audience, and be more engaging and interactive. 
% Additionally, digital services can be more flexible and tailored to the specific needs of a business, and can be updated more easily and quickly.

A  popular form of digital service offered by companies is the \textbf{digital sales channel}. It is an online sales platform that enables businesses to reach and sell to customers through the use of the internet. There are many different types of digital sales channels, such as virtual sales agents, online marketplaces, and social media platforms. Each type of digital sales channel has its own unique advantages and disadvantages that businesses must consider when deciding which channel is right for them. 
Digital sales channels lay within the broader concept of digital marketing which involves applications of digital technologies which form online channels to market, such as web, email, databases, but also mobile and wireless channels and digital TV \cite{chaffey2009internet}.

% \subsection{Businesses deploy chatbots to engage with their target groups}

Chatbots are a great way to engage users. By providing a way for users to communicate with a chatbot, businesses can provide interactive experience that keeps users engaged. Additionally, chatbots can provide a way for users to get information or perform tasks without having to leave the site or app. This can be particularly useful for tasks that are time-consuming or repetitive. 

Businesses may design and deploy chatbots to engage more than one target group of users. Company's customers, vendors, employees and even the public, as often represented by the local community - all may need to be addressed and served by the chatbot. In addition to considering the target group, the design of the chatbot should take into account the specificities of the channel it is meant to address, such as whether it is a text-based or voice-based channel. The design should also ensure that the chatbot is able to answer the different types of queries by different stakeholders that may be directed to it. The success of a chatbot in addressing the needs of its target audience depends on the level of trust that users have on the chatbot. In order for a chatbot to be successful, it is important that users trust the chatbot and believe that it will be able to help them. One of the ways to build trust is to ensure that the chatbot is designed to be transparent and honest with its users.

% In this paper, we focus on the \textbf{conversational agents}, that 
Chatbots become the digital link between the consumer and the company selling the products or services. We mostly address agents from the perspective of customer support. There are several types of consumer oriented virtual agents. To highlight different dimensions of consumer trust, in this paper we mostly think of three types of consumers: streaming service, medical advice service and property sales. Virtual agents may be differentiated by the trust associated dimensions, such as accuracy, language, ethics and other.

\textbf{Virtual sales agents} are a type of digital sales channel that can be used to reach and sell to customers online. Virtual sales agents are automated software programs that are designed to simulate the experience of interacting with a human sales agent. Virtual sales agents interact with customers and provide them with information about a company’s products or services. They can be used to provide customer service, generate leads, and close sales. One of the advantages of using virtual sales agents is that they are available 24/7 and can scale to meet the needs of businesses of all sizes. While they may not be human, businesses are hoping that they will be able to provide consumers with the same level of trust that they would expect from a real salesperson.



% (WHAT'S THIS PAPER ABOUT)
Chatbot is not a human being, hence not subject to the protocols of human interaction, such as in classic understandings of customer engagement or human resources. Characterizing trust in user-chatbot interaction needs novel approaches. This paper discusses the issues of user trust towards chatbots and if chatbot testing can help with user trust. The first chapter provides an overview lays out the environment for the issues of chatbot trust. Key concepts are briefly explained, including digital platforms, digital sales channels, chatbot usage in business settings, virtual sales agents, effectiveness of virtual agents and issues of consumer trust. Overview of the authors previous studies in building chatbots follows. Chatbots of different functions are introduced: 1) a multi-modal educational Rubik's cube chatbot, 2) natural language to structured query (NL2SQL) system, 3) university chatbot and 4) planning chatbot.

In section two, we provide an overview of the terminology and characteristics of business processes in the context of virtual agents. This provides an introduction to the needs and methods for testing chatbots. The need for consumer trust in chatbots is highlighted. Chatbot testing is discussed in section three, where software testing and comparative studies are discussed. The problems of trust related to chatbot under performance is presented. Section four presents three chatbot usage scenarios highlighting unique testing needs for different types of chatbots. Streaming service, medical advice and property sales chatbots are brought as chatbot example applications.

In Figure~\ref{fig:business-setting}, we illustrate the usage of a chatbot in a business setting covering any number of company's products and services. The chatbot is integrated into the company's IT platform which provides an interface for users interaction. Chatbots are designed and launched by the developers who are often hired on a subcontract basis from outside of the company. Chatbots may serve two categories of users - internal and external. Internal users, for example may be the administrators, such as sales staff who receive sales orders and process these. In a business setting, external users are typically company's customers who use chatbot to acquire information about the products and services, but also to submit orders and receive updates about the order. An advanced chatbot processes also customer feedback, complaints and returns.
% -----------------------------------------
 
\begin{figure}[h]
 \centering
   \includegraphics[width=0.7\textwidth]{content/figs/business-chatbot-setting.png}  
   \caption{Chatbot users in a business setting}
   %shown as a decision tree. }
  \label{fig:business-setting}
 \end{figure}
% -----------------------------------------

%\cite{chatbot-testing-tips,chabot-generator} 


\begin{table}[t!]
%\scriptsize
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Chatbot} & \textbf{Domain} & \textbf{Testing Method} & \textbf{Tool Used}  & \textbf{Details}  \\ \hline
ALLURE & Teaching Rubic's Cube (education) & User study & RASA &  \href{https://youtu.be/-0aKDVoEGvs}{Demo},  \cite{allure}
\\ \hline
NL2SQL Bot & Home network (REZERV) /power (MIDAS) info & NA & RASA  & \href{https://vimeo.com/651270271}{Demo},  \cite{t4}
\\ \hline
UniBot & University info & RCTs & RASA & NA 
\\ \hline
PRUDENT & Information retrieval with planning & Unit testing & ParlAI & 
\\ \hline
ElectionBot & Voter information / elections & Focus group & RASA & 
\\ \hline

\end{tabular}
\caption{Different chatbots we built, their domain, testing method, tool used, demonstration link and the relevant papers.}
\label{tab:uofsc-chatbots}
\end{table}

% ------
\subsection{Our Experience in Building Chatbots and Testing Practices Used}

We describe some of the chatbots we have built in different domains and testing methods used.  Table \ref{tab:uofsc-chatbots} gives a summary. 
%We also discuss the testing methods we used to evaluate these chatbots.



% -----
%\subsubsection{Education Chatbot} 
ALLURE \cite{allure} is a multi-modal, collaborative, explainable educational chatbot that is designed to help students to improve their problem solving skills by teaching them how to solve a Rubik's Cube. The chatbot interacts with the users in a multi-modal way by making use of both text and image modalities. It converts output from the black-box Deep Reinforcement Learning (RL) algorithm in the back-end to a human-understandable language and also demonstrates the set of moves the users have to perform using a 3D model of the Rubik's cube on the User Interface (UI). We used RASA \cite{rasa} chatbot framework to build the chatbot and used React JS framework to build the UI around the chatbot. A demo of the system can be found \href{https://youtu.be/-0aKDVoEGvs}{here}. We have conducted a user study to evaluate the chatbot. \kl{Need to add more details about user study.}

%\subsubsection{NL2SQL Chatbot}
NL2SQL chatbot - in \cite{t4}, we built a rule-based natural language to structured query (NL2SQL) system which could convert the Natural Language (NL) query from the user to a MySQL query and fetch the relevant data from the back-end databases. We created a chatbot around this system and implemented it in two different domains with different settings: 
% \begin{itemize}
%     \item 
    {\em Networking:} We used router data in a residence setting. All the internet devices are connected to a smart router that stores and pushes network activity data to the database. 
    %\item 
    {\em Power:} We used IoT power sensor data in a University setting. An electronic sensor is placed in the path of the power source of each device connected to the IoT and data like current and power are captured and pushed to a database. Data was collected from about 100 servers.
%\end{itemize}
We used RASA \cite{rasa} chatbot framework to build the chatbot and deployed it on the Alexa device and a local server for demonstration which can be found \href{https://vimeo.com/651270271}{here}.

\bips{Kausik, put links in Table and describe based on group webpage.}
% \subsubsection{University Chatbot}
% \kl{Need info.}
% \subsubsection{Planning Chatbot}


% \kl{Need info. - Biplav}


==> zip-for-reference-only/content/sec2_background.tex <==
\section{Background}

In this section, we ground the terminology and characteristics of business processes and technology in the context of virtual agents, so that the needs and methods for testing can be better understood.



% -------
\subsection{What are chatbots?}

A chatbot is a computer program that simulates human conversation. It uses artificial intelligence to understand and respond to questions in natural language. Chatbots can range from simple to complex, but most chatbots are designed to perform a specific task, such as customer service or sales.
A simple taxonomy of interaction interfaces we consider {\bf chatbot} for the purpose of the paper is shown in Table~\ref{tab:chatbot-types} under {\em Dimension} column. The {\em users} of the system can be single or a group. As interaction {\em modality}, one can talk to a system or, if speech is not supported, type an input and get the system's response. The system may be for different {\em purposes}: converse in pleasantries without a goal (socialize) and with no need to access data sources, or complete a task like retrieve information or take an action.
To do so, the system can be connected to a static {\em data source} like a company directory or a dynamic data source like disease cases or weather forecast. The application scenarios become more  compelling when the chatbot works in a dynamic environment, e.g., with sensor data,  interacts with groups of people who come and go rather than only an individual at a time, and adapts its behavior to peculiarities of user(s). 
The system can be in many {\em forms} - as software that runs as apps on phones and computers, or embedded into   physical artifacts like kiosks, robots, toys, cars or rooms to give a rich user experience. They may be {\em personalized} to users and be customized for different {\em applications} areas.
This variety is illustrated  in the right column of Table~\ref{tab:covid-decsupport}.

% ---------------------

\begin{table}[t!]
%\scriptsize
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{S.No.} & \textbf{Dimension} & \textbf{Variety} \\ \hline
1 & User & 1, multiple \\ \hline
2 & Modality &  only text,  only speech, multi-modal \\ 
  &   & (input with pointing device, output on a map, ...) \\ \hline
3 & Purpose & socialize, (goal driven:) information seeker,  \\ 
  &  & (goal driven:) delegate action  \\ \hline
4 & Data source & none, static, dynamic \\ \hline
5 & Form & virtual agent, physical device, robot \\ \hline
6 & Personalized &  no, yes \\ \hline

7 &  Domains & general, health, water, traffic, ...\\ \hline

\end{tabular}
\caption{Different Types of Collaborative Interfaces}
\label{tab:chatbot-types}
\end{table}
% ---------------------

 
% --------
\subsection{Business Operations and the Role of Chatbots}

In the past decade, there has been a dramatic shift in the way businesses operate. With the rise of the internet and digital technologies, businesses have had to adapt to a new landscape. This has led to the rise of digital business.

\textbf{Digitalization in business} is the process of using digital technologies to create value for the customers. This can be done in a variety of ways, such as a website, a mobile app, social media or by developing a conversational agent to connect with customers.

Conversational agents gain popularity because it allows to reach a larger audience with the product or service. It also allows the business to connect with customers in a more personal way. Additionally, conversational aagent is more cost-effective than traditional methods of marketing and advertising.

As with traditional customer engagement channels, so do digital channels need to be incorporated into company's general and specific strategies. In case of virtual sales agents, \textbf{digital marketing strategies} need to be addressed. \textbf{Digital marketing} is the process of using the internet and digital devices to promote and sell products or services. Virtual sales agents are only one component in the digital marketing toolbox. Other digital tools, such as  email, social media, search engine optimization, and pay-per-click advertising are also commonly used. A company's digital marketing strategy is be designed to help the company to move towards marketing goals. Hence, digital marketing strategies need to be in line with the overall marketing strategy, but also with the general strategy of the business. Usually, virtual sales agents are complementing other marketing channels to offer a wider selection of customer service platforms. Using any of the customer channels, the goal is to create a customer journey that leads to conversions and sales.

\subsubsection{Chatbot stakeholders}

There are a number of stakeholders within the context of digital business using chatbots as shown in table~\ref{tab:stakeholders}. These include the developers and providers of chatbot technology, the businesses that use chatbots to interact with customers, and the customers themselves. Each of these groups has a different set of interests and needs, which must be considered when developing and deploying chatbots.

\begin{table}
  \caption{Stakeholders of digital business using chatbots}
  \label{tab:stakeholders}
  \begin{tabular}{ |p{3cm}|p{10cm}|  }
    \toprule
    Stakeholder & Interests\\
    \midrule
    \ Developers & Need to ensure that their products are effective and easy to use. They also need to ensure that chatbots are compatible with the systems and platforms that businesses use \\
    \ Businesses & Need to ensure that they are providing a good customer experience. They also need to ensure that chatbots are integrated into their systems and processes in a way that is efficient and effective.\\
    \ Customers & Need to be able to easily find and use chatbots, and they need to be able to trust that chatbots will give them the right information.\\
  \bottomrule
\end{tabular}
\end{table}


 
The increasing availability of new digital technologies has dramatically changed the way businesses interact and communicate with customers. Modern chatbots are utilizing advanced technologies such as artificial intelligence, machine learning, robotic process automation to improve customer engagement. The more complicated chatbots become, the more technologies these deploy, all of which need to be adressed and evaluated in their impact on consumers' trust. Complex chatbots can substitute human service agents in many tasks and can deliver a similar customer experience. Chatbots can fulfill tasks of customer service functions, such as give recommendations, accept orders, process payments, manage shipments, help in troubleshooting and many more. In many cases, chatbots can provide a faster and more convenient experience for users than dealing with a human agent.

% --------
\subsubsection{Methods for Building Chatbots} 

We now review some common ways to build chatbots. 

\noindent {\bf Slot based chatbots}

Slot-based chatbots, also called rule-based chatbots are a type of chatbot that relies on predefined slots to extract information from a user. This information can be used to provide the chatbot with a context for the conversation, or to fulfill a user request. For example, a chatbot may use slots to collect information about a user's travel plans, such as their destination, travel dates, and budget.

\noindent {\bf Learning based chatbots}

Chatbots that are learning based are able to provide a more humanlike interaction than those that are not. These chatbots can keep track of a conversation and provide appropriate responses by utilizing artificial intelligence. This allows for a more natural feeling conversation for the user. Additionally, learning based chatbots can get to know the user over time and provide better recommendations or insights based on the user's preferences.
The main difference from rule-based chatbots is that learning based chatbots can understand inquires and commands that are not recorded in the preset database.

\subsubsubsection{Testing Challenges in Different Approaches}

Slot and Learning based





% ----
\subsection{Software Testing}

Software testing is crucial part of software development. The suggested way to do it is by accounting for it throughout the software development life-cycle. At the specification stage, test plan should be created to check the completeness of the requirements. Then {\em unit testing} should be done as each module is getting completed. Subsequently, {\em system testing } is done during  integration is  followed by  testing  for nun-functional requirements before release of the software. 


% ----
\subsection{The Need for Consumer Trust in  Technology and Chatbots}
In the past, companies could get away with being less than transparent because consumers had no way of knowing any better. Today, however, consumers are more informed and have access to more information than ever before. As a result, companies must pay attentions to their operations, how these impact consumer trust.

There are many factors that contribute to consumer trust. One of the most important is \textbf{transparency}. Consumers need to feel that they can trust the brands they purchase from and that those brands have their best interests at heart. Transparency builds trust between the company and the consumer. If the consumer feels like they can trust the company, they are more likely to engage in business. Transparency also helps to create a positive reputation for the company. If consumers know that the company is open and honest, they will be more likely to recommend it to others. The overall perception of transparency helps to build customer loyalty. 

Chatbots are a way to build consumer trust because they provide an instant, personal connection with the company, including its products and services. Chatbots can answer questions, provide customer support, and even help to elevate the sales of products or services. Chatbots are always there for consumers when they need them and can be trained to address, even to promote the factors of trust, including the transparency.

To make sure if users trust the chatbot, businesses should analyze users profile, which would help avoiding underperformance and shutdown of their chatbot. This can be accomplished, if the
chatbot treats each user based on their corresponding personality profile \cite{muller2019chatbot}.

Another important factor is \textbf{customer service}. If a brand is responsive to customer feedback and complaints, it shows that they care about their customers and are willing to go the extra mile to ensure their satisfaction.

The image of customer service is largely formed by the interactions between customers and customer service representatives. If these interactions are positive, then the customer is likely to have a positive image of customer service. On the other hand, if the interactions are negative, the customer is likely to have a negative image of customer service. 

Technological innovations, such as chatbot based customer service option, may improve the customer experience, when the system is well designed and complements the existing customer service channels. Where call center phone lines may be overloaded, resulting in long waiting times, a well functional customer service chatbot may handle most of the issues, being available 24/7. 

\textbf{Consistency} is another critical determinant of consumer trust. It is important for brands to be consistent. If a brand is constantly changing its message or products, it can be difficult for consumers to trust that they will be getting what they expect. However, if a brand is consistent in its messaging and delivery, consumers are more likely to trust and continue to purchase from them. This why, conservative consumers may alienate from the brand when radical technological changes are affecting their customer experience - such as taking customer service from phone based to a chatbot based servicing. On the other hand, other customer segments may be attracted by the ease of service, when chatbots are introduced. The company needs to know their customer segments and their corresponding service preferences, to make informed and balanced decisions about digital innovations.


==> zip-for-reference-only/content/sec3_trust.tex <==
\section{Trust Problems With Chatbots }

\subsection{Problems of trust}
Chatbot trust issues may resemble trust dilemmas as also related to other customer channels. In case of an incompetent human sales agent, poor quality service may only reflect on the work of one person or a specific case. A badly designed chatbot however, may impact the operations of the entire sales channel. When a chatbot is not designed properly, it may give incorrect or misleading information. This could lead to users making bad decisions based on the chatbot's advice. Additionally, chatbots may not be able to keep up with the pace of conversation, leading to frustrating user experiences. Another issue is that chatbots may not be able to understand a user's emotional state, which could lead to the bot responding in an inappropriate way. Shortcomings in data protections measures, when chatbots may collect personal, which could be used for nefarious purposes.

Depending on the design, chatbots may be easily fooled by humans. Chatbots are computer programs that are designed to simulate human conversation. However, a chatbot may be programmed to respond to a certain keyword with a certain response. If a human user says something that includes that keyword, the chatbot will respond with the programmed response, regardless of the context of the conversation. This can lead to confusion and frustration for the users. Additionally, chatbots may also be fooled by humans using spelling or grammar errors, or by humans deliberately trying to confuse the chatbot. Chatbots may also be intentionally programmed to respond in ways that are not helpful or informative. 

\subsection{Factors affecting users' trust}

\textbf{User trust} is a multifaceted issue involving accuracy, privacy and other issues of user engagement with any chatbot. A chatbot may not be able to accurately understand or respond to the user's needs. Additionally, chatbots may not be able to keep user information confidential, which could lead to privacy issues.

As digital platforms become prevalent in business services, companies must be aware of how their digital channels affect consumer trust. Consumers are increasingly likely to research a company and its products online before making a purchase, and their trust in a company can be heavily influenced by their online experiences. A company's digital channels provide an opportunity to build trust with consumers by providing accurate and up-to-date information, being responsive to customer inquiries, and maintaining a strong online presence. Conversely, a company's digital channels can also damage consumer trust if they are neglected or poorly managed. It is therefore essential for companies to carefully consider how their digital channels can impact users' trust.

It is essential for businesses to build trust with their users in order to improve customer loyalty. By establishing trust, businesses can create a loyal customer base that will continue to use their products and services.
Trust towards digital platforms may play a critical role in the operational success of said platforms. In other words, if users don't trust a platform, they're less likely to use it. This could lead to a decrease in usage of the platform and consequent loss of revenues. 
Additionally, user trust is important for platforms because it can help to create and maintain brand loyalty. Users who trust a platform are more likely to be loyal to the brand and recommend it to others.

There are many factors that affect \textbf{consumer trust}. Some of these include the company’s reputation, its transparency, its customer service, and its return policy. Other factors include the company’s communication style, the design of its digital channels, and the reviews that consumers can find online from other consumers. Ultimately, it is up to the consumer to decide how much trust to place in a company. Consumer trust is essential for the success of digital sales channels. When consumers feel they can trust a company, they are more likely to do business with them. This trust can be built through transparency, providing accurate information and delivering on promises. Creating a strong relationship of trust with customers can help ensure long-term success for a company.

An \textbf{effective virtual agent} creates trust in consumers by providing accurate and up-to-date information about the products or services they are interested in. They are also transparent about their company’s policies and procedures, and are quick to respond to any questions or concerns that consumers may have. In addition, virtual agents are typically very personable and easy to communicate with, which helps build rapport and further instills confidence in the consumers they are assisting. Ultimately, by being knowledgeable, responsive, and friendly, virtual agents are able to successfully build trust with consumers, leading to satisfied customers and repeat business.

There are a few key factors that contribute to a \textbf{chatbot's competence}. A chatbot must be able to understand the user's input. This is achieved through natural language processing (NLP). Once the chatbot understands the user's input, it must be able to generate a response that is relevant to the user's inquiry. This requires a knowledge base that the chatbot can draw from to generate an appropriate response.  The more detailed database, the higher is the perceived competence of a chatbot. The more accurate the chatbot is in its understanding of the user input and the more relevant the response, the more trust the user will have in the chatbot.

\subsubsection{Accuracy}
Chatbots are not always accurate. The better trained chatbot, the more accurate performance. However, most chatbots are imperfect in their training and are adequately responding only to a limited number of intents. A chatbot with more intents is able to handle more varied user input. This means that the chatbot can respond to a wider range of user queries, which can be helpful in terms of providing a better user experience. Additionally, a chatbot with more intents is likely to have more training data, which can help to improve the chatbot's performance. Chatbot with more intents is more likely to be able to handle edge cases, which can again improve the user experience.

\subsubsection{Reliability} is another key factor in chatbot effectiveness. Businesses deploying chatbots, are trusting the artificial intelligence to carry out conversations on their behalf. A reliable chatbot is designed and and trained to handle most of users' requests. A chatbot that is designed well will be able to understand human conversation and respond accordingly. It will also be able to handle different types of input, such as natural language, text, and even voice. A chatbot that is well-trained will be able to carry out conversations more smoothly and accurately. It will know how to respond to different types of questions and requests, and it will be able to handle different types of conversations.

\subsubsection{Transparency} is a critical part of reliability directly impacting users' trust. Revealing their artificial identity is a central question for any chatbot and customer interaction. A well integrated chatbot provides a seamless customer experience and improves customer satisfaction. Such a chatbot works in line with other tools and channels as deployed by the company and all aimed at providing a trustworthy experience. A transparent chatbot will reflect the transparency of the business in its dealings with customers, providing them with clear and concise information about its products and services. A transparent company is responsive to customer queries and concerns, and always acts in the best interests of the customer. By adhering to these principles, a company can build a chatbot reflecting this trust with its customers, resulting in a long-lasting relationship of mutual respect and understanding.

\subsubsection{Use of language}
A chatbot might use profanity, make threatening comments, or engage in other forms of verbal abuse. This type of language is not only hurtful, but can also be illegal. Abusive language can have a significant impact on chatbot trust. By using profanity or other offensive language, users can create a negative association with the chatbot that can dissuade others from trusting it. In some cases, abusive language can also lead to chatbot technical issues. As such, it is important to be mindful of the language used when interacting with chatbots, in order to maintain a positive relationship and avoid any potential negative impacts.
Chatbots that use profanity can give users a negative impression of the chatbot and the company or organization that chatbot represents. Additionally, profanity can also be seen as a sign of disrespect towards the users of the chatbot. If chatbots continue to use profanity, it is likely that they will eventually be shut down.

\subsubsection{Response time}
Chatboth's response time and time to reach a resolution can also impact the reliability. When a chatbot is slow to respond and reach a satisfying resolution, this can be a source of frustration for customers who are trying to get help or information. As with any customer service interaction, response time and resolution time are key factors in chatbot reliability and customer satisfaction. If a chatbot is taking too long to respond to queries, or is unable to resolve issues in a timely manner, customers will likely  look for alternatives ways for getting the needed information or reach another form of resolution. On the other hand, chatbots that are able to quickly and efficiently resolve customer issues will foster trust and satisfaction. In order to maximize chatbot reliability and customer satisfaction, businesses should monitor response and resolution times closely, and make improvements as needed.

Studies have shown that people are more likely to trust a technology if it is perceived to be reliable. If chatbots are perceived as unreliable, this could lead to decreased trust in the technology overall. This could have a negative impact on how people view chatbots and could lead to fewer people using them.
Chatbots reliability can be undermined by many ways. Overall, a competent and reliable perception of a chatbot is important for ensuring that its able to carry out conversations effectively and accurately, hence gaining trust of the users. 



==> zip-for-reference-only/content/sec4_chatbottesting.tex <==

\section{Chatbot Testing Methods}

After launching a chatbot, the company needs to monitor \textbf{ chatbot's performance} and to determine if it's performing optimally and achieving company's goals. From the perspective of users' trust, the chatbots performance is mainly related to its competence and reliability. Performance metering can be done through a variety of methods, such as tracking key metrics, conducting user surveys, and A/B testing. By doing so, the company can identify areas for improvement and make necessary changes to ensure the chatbot is providing the best possible experience for users.

\subsection{Purpose and types of tests}
Chatbot testing is the process of testing a chatbot to ensure it is functioning correctly and providing an accurate and consistent experience for users. By testing, companies can identify any issues that need to be addressed, such as incorrect responses, errors, or slow performance. Testing also allows to fine-tune chatbot's design and functionality, as well as assess its overall effectiveness. This involves testing the chatbot's ability to understand and respond to user input, as well as its overall functionality. Chatbot testing can be performed manually or using automated software testing tools.

Testing may include, assessing how well the chatbot understands customer queries, how accurate the chatbot's responses are, and how satisfied customers are with the chatbot experience. Customer satisfaction is one of the key factors of chatbot effectiveness.

\subsection{Software testing}
Chatbot software testing is an important part of the development process, as it helps to ensure that the chatbot is able to deliver a good user experience. 

Chatbot testing can be approached as any other software testing. These methods include unit testing, integration testing, system testing, and acceptance testing. Unit testing is the testing of individual chatbot components, while integration testing is the testing of how those components work together. System testing is a more holistic approach that tests the entire system, including the connections to databases, such as customer, orders, inventory and other. 

Chatbot software testing is essential to ensure that chatbot functions as intended and provides a positive experience for users. Chatbot functional testing ensures that the chatbot is able to handle all the different types of input that it may receive and provide the appropriate responses. Load testing ensures that the chatbot can handle high volumes of traffic without experiencing any issues.

\subsection{Testing as Software Systems}

\subsection{Testing as AI}

\subsubsection{Data sources and provenance}

Data provenance is the origin of data and the history of how it has been transformed over time. Data provenance is often used to track the origins of data, to ensure that it has not been tampered with, and to verify its accuracy. In many cases, data provenance can be used to trace the path of data from its inception to its current form.

As chatbots increasingly become relied upon to handle larger amounts of data, data provenance will become an increasingly important factor in their design and function. Data provenance refers to the origin and history of data, and how it has been transformed over time. For chatbots, data provenance affects how they handle data, what data they have access to, and how that data is used.

Chatbots rely on data to function. If the data they are using is of poor quality or unreliable, the chatbot will be less effective. Data provenance can affect the chatbot’s decision-making. If the chatbot is not aware of the provenance of the data it is using, it may make decisions that are not in the best interest of the user. 

\subsubsection{Large language models (LLMs)}

Large language models (LLMs) are a type of artificial intelligence that are used to process and understand natural language. These are neural networks that are trained on a very large corpus of text. The models are able to learn the statistical properties of the language and can generate text that sounds like it was written by a native speaker. The models are also very good at understanding the context of a sentence, which allows them to generate more natural sounding text. For example, if you ask a chatbot about the weather, it can provide you with information about the current weather conditions as well as the forecast for the next few days.
LLMs can be used for a variety of tasks, including machine translation, question answering, and text classification.

\subsection{Testing as a Decision Support Tools (Comparative Studies)}
Comparative studies are a form of usability testing that assesses how easy it is for users to interact with the chatbot. A comparative study is a effectiveness determination method that observes, if needed, intervenes and compares two or more subsamples, to to identify similarities and differences. This research method can be used to compare anything from individuals to entire organizations. When conducting a comparative study, it is important to control for as many variables as possible in order to create a fair comparison. Once the data is collected, it must be analyzed in order to identify any patterns or trends.
The most reliable way to test the effectiveness of a chatbot is through comparative studies. The most commonly used forms of comparative studies are before/after, case-control, A/B testing and randomized control trials (RCT). There are some important differences between these two types of study designs. A/B testing is designed to test which chatbot works best, while a randomized control trial looks at why it works best. 
In this study we discuss two afore mentioned testing methods, as these are most commonly used and are most advanced and reliable methods for testing for trust.

\subsubsection{A/B testing}
A/B testing is a method of experimentation in which two versions of a chatbot are shown to users at random, and statistical analysis is used to determine which version is more effective. This technique can be used to test anything from chatbot copy to virtual agents capable fullfilling all the tasks of human agents. It also can be used to evaluate how effective a chatbot or virtual agent is in comparison to human agent.
This technique is especially useful when testing or evaluating chatbots because it can help isolate the specific areas where the chatbot falls short. For example, if a chatbot is not able to properly handle customer inquiries, this technique can help identify that particular issue. Additionally, this technique can also be used to evaluate how well a chatbot or virtual agent performs in comparison to human agents.

\subsubsection{Randomized controlled trials}
Randomized controlled trials are a type of scientific experiment that are used to test the effectiveness of a new treatment or intervention. For example, a treatment is a new chatbot, whereas a control is an old chatbot. Industries' best standard or a competitors chatbot could also serve as a control. Additionally, the company to compare a chatbot against other information acquisition channels, such as customer service call center.  The participants in a randomized controlled trial are randomly assigned to either the group receiving the new treatment (a new chatbot) or the control group receiving the standard treatment (an old chatbot). The two groups are then compared to see if the new treatment is more effective. Randomized controlled trials are considered the gold standard of scientific evidence. However, in the case of chatbots, there is a lack of high-quality evidence to support claims of effectiveness, as most chatbot studies do not deploy RCT. RCT is a resource demanding study method that requires time money and often a large number of human test subjects. A recent systematic review found that only two out of eleven studies meets the criteria for an acceptable randomized controlled trial. The other nine studies were either non-randomized or had important methodological flaws. 





==> zip-for-reference-only/content/sec5_testing_commplatform.tex <==
\section{Case Study: Chatbot Testing Support in Open and Commercial Platforms}


\subsection{Review of Current Practices}

\bips{Nice if we can have a table with references to testing guidance from different vendors. Open Source - parl.ai, rasa, mindmeld.
Keywords: testing, testing guidelines, development process, release checklist}
Chatbots are built for control. Not data-driven ?


\subsubsection{Testing in Watson}
\bips{Sachin - please add based on IBM platform over the years, and coming up.}

\subsubsection{Testing in Rasa}

\subsubsection{Testing in ChatGPT}


\subsection{Testing for Intent Detection}

\begin{itemize}
    \item Handling out-of-scope
\end{itemize}

\subsection{Testing for Actions to Be Taken for an Intent}


\subsection{End-to-end Testing}

Some services provide regression but they are not guaranteed for anything.. Botium. 

\subsection{Opportunities to Improve}

Hate Speech detection. 





==> zip-for-reference-only/content/sec6_usagescenarios.tex <==

\section{Usage Scenarios - Applications and Unique Testing Needs}

In this chapter we focus on three use cases, discussing the characteristics of those and how these affect chatbot's trust-

Table~\ref{tab:freq} is included in the input file; compare the
placement of the table here with the table in the printed output of
this document.

\begin{table}
  \caption{Overview of chatbot use cases and related trust issues}
  \label{tab:freq}
  \begin{tabular}{ |p{2.5cm}|p{2.5cm}|p{2.5cm}|p{6cm}| }
    \toprule
   Use case&Age of the user&Investment&Focus of user trust\\
    \midrule
    \ Streaming service& Adult and adolescent& Low&Mostly related to protecting adolescents from adult content.\\
    \ Medical advice& Adult& Medium&Related to the health and well-being of the patient.\\
    \ Property sales & Adult & High&Related to transparency and objectivity in investment recommendations.\\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Streaming service chatbot}
In the example  of a streaming service, like Netflix, a chatbot helps the user to find the right movie to watch on their subscription platform. It asks the user questions about what categories they like and don't like, and asks for favorite movies, shows. The chatbot recommends movies for the user.

Movie recommendation is probably one of the lowest personal or property liability examples for a chatbot. However, adult content needs to be screened and made inaccessible for adolescents. A trusted movie chatbot would be capable of identifying the age of the user and accounting for that in its movie recommendations. Besides recommending the titles, the chatbot also needs to account for the language, as it should consider the age of the user.

\subsection{Medical advice chatbot}
Medical advice chatbots are becoming increasingly popular as a way to provide quick and easy medical advice. They are typically used to answer basic questions about medical conditions and treatments, and can be accessed through a chat interface on a website or mobile app.

Medical advice chatbots are needed to be powered by AI models, which allows them to understand natural language queries and provide accurate responses. In some cases, chatbots may also be able to provide personalized recommendations based on a user's individual symptoms or health condition.

So far, due to the risk of liability of malpractice, no chatbot is able to substitute  a human doctor. 
Medical chatbots are subject to highest personal liability, as the function of such service would result in an outcome of human health. Such chatbots need to be able carry the functions of a human doctor, including understanding the health history of the patient, dispositions and side effects and accumulative effects of the medicine. When a chatbot that would prescribe medicine would also need to account for the accumulative effect of multiple prescriptions. 

Seitz et al. studied diagnostic conversational agents. They found that interpersonal trust approaches do not fully explain the build up of trust to diagnostic CAs. Communicative aspects are important in chatbot interactions, but users don't expect a CA to fulfil social needs. Transparent handling of information and justifications are important to build up trust since trust mostly arises cognitively while underlying the technical character of agents. Besides afore mentioned, also  more natural conversation can substantially play a role in trust development. The study identified six trust-building factors in diagnostic chatbots - purpose, reliability, interface design, interaction capabilities, transparency and relativization.  \cite{seitz2022can}

\subsection{Property sales chatbot}

A Property Sales chatbot is a chatbot that is designed to help people with the purchase or sale of their property. The chatbot will ask the user questions about their property or the desired property, such as the price range, the location, and the number of bedrooms. The chatbot will then provide the user with a list of potential buyers or estimate the sales price. 
Property chatbot entails a high expenditure, which makes any misinformation given by the chatbot open for a liability claim. High responsibility requires highest levels of trust in the eyes of the users.
Additionally, chatbot may be required to ckeck the buyer's credit score in order to validate the purchase request. A mortage can not be advised by the chatbot if the buyer is likely incapable of servicing the loan.

Mozafari et al. studied chatbot trust with respect to customer retention. They found that if the chatbot is successful in solving customers' issues, disclosing the identity of chatbot will negatively impact customer trust and therefore obstruct retention for highly critical services. Otherwise, for services of less critical nature, chatbot disclosure won't impact trust. The deficit of trust comes from lower perceptions of agent's competence and benevolence. Lowe benevolence is attributed to perceived lower empathy Agents that are disclosed as virtual agents are seen as less knowledgeable. \cite{mozafari2021trust, bhattacherjee2012user}

==> zip-for-reference-only/content/secx_others.tex <==


\section{Discussion}


\subsection{Additional Content from Intro}


\subsection{Discussion Content}

Chatbot trust is a complex issue which requires correspondingly complex approach. A trusted chatbot should be adaptive to users need and take into account their personal background. 
Müller et al. determined different user profiles of personality traits to indicate their relative differences of their ability to trust chatbots. They identified three basic personality profiles and their relative level of trust - introverted careless distrusting user, conscientious curious trusting user, careless dishonest trusting user. The user profiles should suggest how the chatbot treats users to result in a perceived trust experience.\cite{muller2019chatbot}

Przegalinska et al. recommended companies focusing on three trust-enhancing features: transparency, integrity, explainability. Transparency means sending signals of honesty in communication, and does not deny its status. Agent also needs to be predictable. The trustors (users) expect that an agent, an object of trust, would act consistently in line with past experience. User perceiving  chatbots as predictable, leads to perception of trust towards the chatbot \cite{przegalinska2019bot}.

What more is needed

\section{Conclusion}

In order to motivate a chatbot for customer interaction it is important to keep the \textbf{chatbot's goals} in mind and make sure that they are aligned with the company's goals. This is is best done before designing a chatbot. Any chatbot's goals should match with  company's goals. Chatbots should be designed to contribute to specific operations and to help the company achieve its desired performance. To do this, first company's specific goals related to the chatbot tasks are identified. These goals are then matched with the features and capabilities of various chatbot strategies. 



